Sky2Ground: A Benchmark for Site Modeling under Varying Altitude

We introduce Sky2Ground, a three-view dataset designed for varying altitude camera localization, correspondence learning, and reconstruction. The dataset combines structured synthetic imagery with real, in-the-wild images, providing both controlled multi-view geometry and realistic scene noise. Each of the 51 sites contains thousands of satellite, aerial, and ground images spanning wide altitude ranges and nearly orthogonal viewing angles, enabling rigorous evaluation across global-to-local contexts. We benchmark state of the art pose estimation models, including MASt3R, DUSt3R, Map Anything, and VGGT, and observe that the use of satellite imagery often degrades performance, highlighting the challenges under large altitude variations. We also examine reconstruction methods, highlighting the challenges introduced by sparse geometric overlap, varying perspectives, and the use of real imagery, which often introduces noise and reduces rendering quality. To address some of these challenges, we propose SkyNet, a model which enhances cross-view consistency when incorporating satellite imagery with a curriculum-based training strategy to progressively incorporate more satellite views. SkyNet significantly strengthens multi-view alignment and outperforms existing methods by 9.6% on RRA@5 and 18.1% on RTA@5 in terms of absolute performance. Sky2Ground and SkyNet together establish a comprehensive testbed and baseline for advancing large-scale, multi-altitude 3D perception and generalizable camera localization. Code and models will be released publicly for future research.Project page: https://sky2ground2026.github.io/sky2ground/

==> sections/0_abstract_short.tex <==
\begin{abstract}
We introduce Sky2Ground, a three-view dataset of 51 sites designed for multi-altitude camera localization and reconstruction across satellite, aerial, and ground perspectives. By combining structured synthetic imagery with real, "in-the-wild" data, we provide a rigorous testbed for evaluating global-to-local contexts under varying altitudes. Benchmarking state-of-the-art models like DUSt3R and VGGT reveals that satellite imagery often degrades performance due to significant altitude shifts and sparse geometric overlap. To address these challenges, we propose SkyNet, a two-stream architecture that utilizes Masked-Satellite-Attention (MSA) and a curriculum-based training strategy to progressively integrate satellite views. SkyNet significantly improves cross-view consistency, outperforming existing methods by 9.6\% on RRA@5 and 18.1\% on RTA@5. Code and models will be released for future research.
\end{abstract}


==> sections/1_intro_short.tex <==
\begin{figure*}[t]
  \centering
  \vspace{-2em}
  \includegraphics[width=1\linewidth]{figs/data_example.png}
  \caption{\textbf{Cross-view examples from the Sky2Ground dataset.} Satellite, aerial, and ground-level images for a variety of urban scenes in Sky2Ground, where each column corresponds to a unique site. These examples highlight strong viewpoint and appearance variations across modalities, revealing the challenges of cross-view matching and multi-scale scene understanding. Real images additionally introduce diverse lighting conditions, weather effects, and natural scene noise, further emphasizing the complexity of real-world cross-view perception.}
  \label{fig:data}
  \vspace{-1em}
\end{figure*}

\section{Introduction}
\label{sec:intro}

Jointly localizing multi-view images and constructing reliable 3D models is a fundamental task with diverse applications, including geo-registering ground-images~\citep{mithun2023cross,pittaluga2019revealing,workman2015wide}, outdoor-scene reconstruction~\citep{patel2020visual,rezaei2024sat2map,argota2025urban}, urban-view synthesis \cite{xiangli2022bungeenerf,xu2023vr,li2023matrixcity,lehtola2022digital}, and complex navigation~\citep{mithun2023cross,li2024learning,peldon2024navigating}. While classical pipelines like COLMAP~\cite{schoenberger2016mvs,schoenberger2016vote} rely on computationally intensive heuristics, recent neural networks enable faster geometry inference through pre-training on ground-aerial datasets \cite{mast3r_arxiv24,dust3r_cvpr24,wang2025vggt,vuong2025aerialmegadepth}. However, modeling large-scale scenes across multiple altitudes—specifically incorporating satellite imagery—remains underexplored.

Unlike ground/aerial views, satellite imagery provides globally consistent coverage and stable geospatial reference frames~\citep{mari2022sat}. Despite its utility for UAV localization from oblique perspectives~\citep{patel2020visual,mari2022sat,conte2008integrated}, no existing work focuses on the joint-localization of cameras across ground, aerial, and satellite views simultaneously. Motivated by the goal of planet-wide reconstruction \cite{vuong2025aerialmegadepth}, we propose \textbf{Sky2Ground}: a multi-altitude, cross-view dataset that unifies synthetic satellite, aerial, and ground imagery with real images collected ``from-the-wild''. The synthetic component provides dense, consistent camera poses, enabling a thorough evaluation of cross-view pipelines.

Our benchmark reveals that existing pose estimation methods struggle with the distributional shifts of satellite imagery. While aerial and ground modalities reinforce each other, a single satellite image can destabilize training, highlighting the challenges of multi-altitude integration. To address this, we introduce \textbf{SkyNet}, a two-stream architecture featuring: 1) a \uline{G}round-\uline{A}erial-\uline{S}atellite (GAS) encoder with \uline{M}asked-\uline{S}atellite-\uline{A}ttention (MSA) that prevents aerial/ground modalities from interacting with satellite features; and 2) a dedicated Sat-Encoder for explicit satellite processing. SkyNet utilizes curriculum-based strategies—gradually sampling distant views and using aerial images as a ``bridge''—to adapt and improve upon models like VGGT while retaining the advantages of large-scale pre-training.

Our contributions are summarized below:
\begin{enumerate}
    \item \textit{Sky2Ground Dataset}: A large-scale dataset integrating satellite, aerial, and ground-level imagery with both synthetic and real components, providing annotations for camera poses and dense depth maps.
    \item \textit{First Benchmark}: A comprehensive study of existing methods on joint cross-view localization and reconstruction involving all three ground/aerial/satellite imagery.
    \item \textit{SkyNet Architecture}: A single-forward pass model that outperforms DUSt3R, MASt3R, Map-Anything, and VGGT on cross-view localization.
\end{enumerate}


==> sections/2_related_short.tex <==
\section{Related Works}
\label{sec:rw}

\noindent \textbf{Cross-View Camera Localization:} requires inferring camera poses (intrinsics/extrinsics) across aerial, ground and satellite views. Classical SfM pipelines like Colmap \cite{schoenberger2016mvs,schoenberger2016sfm} face issues in matching-features across such diverse-viewpoints. Additionally, the large-scale of captured images and their varying-altitude further exacerbates this problem. Other works \cite{dust3r_cvpr24,mast3r_arxiv24,hu2022beyond} instead learn canonical-transformation between a pairs of views via neural-nets. However, they require an additional global-alignment phase to map all prediction-pairs onto a consistent point-map representation. Recently, VGGT \cite{wang2025vggt} has shown that a single-forward pass through transformer is enough to infer camera parameters. In this work, we observe that simply fine-tuning VGGT on combination of ground/aerial/sat views hurts performance. We propose an alternate method named \textbf{SkyNet}, which we hope is a small-step towards fixing this non-trivial problem.

\noindent \textbf{Cross-View and Novel-View Synthesis:} Recent advances in Neural Radiance Fields (NeRF) \cite{mildenhall2021nerf} and Gaussian Splatting \cite{kerbl20233d} have significantly improved cross-view and novel-view synthesis across diverse capture settings. Several methods leverage aerial imagery \cite{tang2025dronesplat, xiangli2022bungeenerf, zhang2025birdnerf, chen20253d, wu20243d, yuan2025robust, gao2025citygs, liu2024citygaussian, liu2024citygaussianv2} to model large-scale scenes \cite{somanath2024towards,kikuchi2022future}, while hybrid approaches combine aerial, and ground viewpoints to enhance coverage and geometric stability \cite{jiang2025horizon, zhang2025crossview, joshi2025unconstrained, ham2024dragon,zhai2017predicting,modi2023occlusions}. Some works \cite{xiangli2022bungeenerf, liu2024citygaussian} incorporate level-of-detail representations, whereas others \cite{zhang2025crossview} fuse separate sub-models for aerial and ground views. Progressive strategies such as Dragon \cite{ham2024dragon} gradually integrate images captured from different altitudes to stabilize reconstruction. In contrast, our method performs a unified, full-scale reconstruction that jointly integrates aerial, ground, and satellite observations.

\begin{table}[ht!]
\centering
\caption{Comparison with existing datasets. A: Aerial, G: Ground, Sat: Satellite, Syn: Synthetic.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Dataset} & \textbf{Sites} & \textbf{Imgs}  & \textbf{Syn A} & \textbf{Syn G} & \textbf{Real A} & \textbf{Real G} & \textbf{Sat}  \\
\midrule
KITTI-360 \cite{liao2022kitti}        & 1  & 300k   & \ding{55} & \ding{55} & \ding{55} & \checkmark & \ding{55}  \\
nuScenes \cite{caesar2020nuscenes}    & 2  & 1.4M  & \ding{55} & \ding{55} & \ding{55}  & \checkmark & \ding{55}  \\
GauU-Scene \cite{xiong2024gauu}       & 6  & 4.7k   & \ding{55}  & \ding{55} & \checkmark  & \ding{55} & \ding{55}  \\
UC-GS \cite{zhang2024drone}           & 2  & 1.4k     & \checkmark & \checkmark & \ding{55}  & \ding{55} & \ding{55}  \\
BungeeNeRF \cite{xiangli2022bungeenerf} & 12 & 3.1k   & \checkmark & \ding{55} & \ding{55}  & \ding{55} & \checkmark  \\
MatrixCity \cite{li2023matrixcity}    & 1  & 519k      & \checkmark & \checkmark & \ding{55}  & \ding{55} & \ding{55}  \\
AerialMegaDepth \cite{vuong2025aerialmegadepth}    & 137  & 132k       & \checkmark & \checkmark & \ding{55}  & \checkmark  &  \ding{55} \\
\midrule
\textbf{Ours}                         & \textbf{51} & \textbf{80k}  & \checkmark & \checkmark & \checkmark  & \checkmark & \checkmark \\
\bottomrule
\end{tabular}}
\label{tab:custom_comparison}
\end{table}

\noindent \textbf{Public Datasets:} In Tab. \ref{tab:custom_comparison}, we compare across existing datasets. nuScenes \cite{caesar2020nuscenes} and KITTI-360 \cite{liao2022kitti} are autonomous-driving datasets and lack aerial/satellite views. Similarly, AerialMegaDepth \cite{vuong2025aerialmegadepth} contains ground/aerial views but lacks satellite-views. Synthetically-rendered datasets like MatrixCity or BungeeNeRF remain limited to synthetic scenarios. In contrast, Sky2Ground covers all three viewpoints, as well as manually-scraped real ground/aerial views. To our knowledge, no prior-work offers a comprehensive dataset across all three viewpoints with both real/synthetic images and an in-depth study of their impact.


==> sections/4_method_short.tex <==
\section{Sky2Ground Dataset}
\label{sec:dataset}

Sky2Ground is a diverse dataset comprising $80k$ images across $51$ global locations, providing unified synthetic and real-world views from satellite, aerial, and ground perspectives. As shown in Fig. \ref{fig:drone}, the dataset spans the globe to ensure geographic diversity. Each site includes synthetic satellite imagery (1--2 km altitude), aerial views (200--800 m), and ground-level captures (5--80 m). To introduce realistic lighting, weather, and noise, we manually curate real-world imagery from Google Maps and YouTube. We provide dense depth-map annotations and camera intrinsics/extrinsics for all images.

\begin{table}[H]
\centering
\caption{Sky2Ground dataset statistics. A: Aerial, G: Ground, Sat: Satellite, Syn: Synthetic. -: altitude for real is unknown.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Attribute} & \textbf{Sat} & \textbf{Syn A} & \textbf{Real A} & \textbf{Syn G} & \textbf{Real G} \\
\midrule
Modality         & Ortho-Rectified & RGB  & RGB  & RGB & RGB \\
\#Images per site        & 120   & 1080 & 120 & 50--250 & 120\\
Altitude (AGL)   & 1--2 km & 200--800 m & - & 5--80 m & -\\
\bottomrule
\end{tabular}}
\label{tab:tier_overview}
\end{table}

\noindent \textbf{Collection and Annotation:} Synthetic data is collected via Google Earth Studio using specific trajectory paths: a circular walk-around for ground views, top-down sampling for satellite views, and a virtual triple-camera rig following a downward helical trajectory for aerial views. Satellite images undergo ortho-rectification to correct perspective distortions. Aerial imagery is captured across three altitude bands (800 m, 500 m, and 250 m) to ensure multi-scale coverage. To provide dense supervision required for models like VGGT \cite{wang2025vggt}, we generate depth maps by running a dense-MVS pipeline via ColMAP on the synthetic poses, utilizing PatchMatch Stereo and Stereo-Fusion for robust geometry estimation.

\begin{figure*}[t!]
  \centering
  \vspace{-2.5em}
  \includegraphics[width=0.92\linewidth]{figs/overview.png}
  \caption{\textbf{Overview of the Sky2Ground dataset.} The middle trajectory illustrates camera poses from one of our collected sites. Dots indicate ground-truth camera positions for synthetic images, while red frustums represent the estimated camera poses for real images. The surrounding images showcase example satellite, aerial, and ground views—where the real images demonstrate more diverse illumination conditions and realistic noise. The top-right map depicts the geographic distribution of all collected landmarks, highlighting the dataset’s global coverage.}
  \label{fig:drone}
  \vspace{-2em}
\end{figure*}


==> sections/5_exp_short.tex <==


\section{Sky2Ground Benchmark}
Here we present Sky2Ground Benchmark where we evaluate existing models for camera localization/rendering-based tasks. We describe the experimental setup, and then present additional analysis. 

 \begin{figure}[ht!]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/benchmark_split.png}
    \vspace{-0.8em}
    \caption{\textbf{Benchmark splits and modality setups.}
  (a) Image counts per split for synthetic CR - Core, D1 - Dense 1, D2 - Dense 2, D3 - Dense3 and D4 - Dense 4, across ground, aerial, and satellite views.
  (b) View combinations used in each benchmark setup: Ground (G), Ground+Aerial (GA), Ground+Satellite (GS), and Ground+Aerial+Satellite (GAS).
  }
     \vspace{-2.0em}
    \label{fig:benchmark split}
\end{figure}

\indent \textbf{Experimental setup:}
In Fig.~\ref{fig:benchmark split}, we show that our dataset comprises of five synthetic splits (CR, D1–D4). Here D1–D4 provide progressively denser-image coverage. Note that core images, (CR) are \textit{common} to all the splits, i.e. (CR, D1-D4). We analyze existing methods on $D2$ setup. We \textit{evaluate} on a subset of $D2$ images, i.e. the core-setup $CR$. This ensures that although the \textit{total number} of images across $D1-D4$ changes, evaluation setup \textit{stays consistent}. Additionally, we evaluate various gaussian-splatting methods for scene-rendering. Therefore, our analysis covers \textit{both} localization/rendering.\\
\indent \textbf{Models.} We benchmark a wide variety of \textit{learning-based} methods for camera-localization. For eg, we evaluate \textit{pair-wise view processing} nets like Dust3r/Mast3r/MapAnything. Additionally, we evaluate \textit{VGGT} which infers camera-poses in a single feed-forward. Additionally, we benchmark classical SfM techniques like COLMAP, and provide more results in the supplementary. For rendering, we evaluate models like %
2DGS, 3DGS, and 3DGS-MCMC, which span 2D splatting, 3D Gaussian scene representations, and an MCMC-refined 3D variant.\\
\indent \textbf{Metrics:} We evaluate camera-localization performance via Relative Rotation Accuracy (RRA) and Relative Translation Accuracy (RTA)~\citep{Jin2020rrarta}. More specifically, we threshold at $5^\circ$, and report RRA@5$^\circ$/ RTA@5$^\circ$. This denotes, how well the model localizes cameras within $5^\circ$ of each-other. We quantitatively evaluate photometric/perceptual quality of 3D-renderings via PSNR and DreamSim metrics. A higher value of PSNR is assumed better, whereas for DreamSim \textit{lower-score} is better. 


\subsection{Zero-shot Analysis}
Here, we first discuss about \textit{zero-shot} localization performance of existing models, and variation as number of input views changes. Next, we discuss rendering results. 

\begin{figure}[ht!]
    \centering
    \vspace{-1em}
\includegraphics[width=0.95\columnwidth]{figs/figure4.pdf}
    \caption{
    Comparison of \textbf{RRA@5} and \textbf{RTA@5} metrics for four methods 
    (Dust3r, Mast3r, Map Anything, and VGGT).
    }
    \label{fig:rra_rta_lineplots}
    \vspace{-1em}
\end{figure}

\indent \textbf{Models `suffer' when number of views are less}: In Fig.~\ref{fig:rra_rta_lineplots}, we plot how $RRA/RTA$ varies  as the number of input views increases $core\rightarrow dense1 \rightarrow dense2$. We observe models perform \textit{worse} on sparse scenarios, i.e. \textit{core}. \\
\indent \textbf{VGGT performs best on Ground/Aerial setup:} We note that VGGT (purple-curve) performs best on Ground/Aerial scenarions. One notable thing is that performance of VGGT \textit{does not fluctuate} much as compared to Dust3r/Mast3r/Map-Anything, indicating that it does well in \textit{sparse-scenarios.}\\
\indent \textbf{Pair-wise view networks like Dust3r do well on satellite}: In Fig.~\ref{fig:rra_rta_lineplots}, we note that Dust3r achieves highest performance on localizing \textit{satellite} images (red curve). We believe that this is due to \textit{global-alignment} enforced in dust3r. Satellite-views contain a lot of mutually-common points, and an explicit matching step ensures proper alignment. However, we note that Dust3r/Mast3r \textit{don't} perform well on \textit{ground} scenarios. \\



\begin{figure}[ht!]
    \centering
    \vspace{-2em}
\includegraphics[width=\columnwidth]{figs/g_ga_gs_gas.pdf}
    \caption{
    Comparison of models across view combinations.
    }
    \vspace{-1em}
    \label{fig:g_ga_gs_gas}
\end{figure}

\noindent \textbf{Satellite images pose a `significant-problem':} One expectation might be that models  \textit{ should perform better} on ground+aerial+satellite (GAS) setup than ground+aerial setup, because adding satellite provides more information to the neural-net. In Fig\ref{fig:g_ga_gs_gas}, we surprisingly find that this \textit{is not} the case. Instead, we observe \textit{drops} in performance. Therefore, processing \textit{satellite} modality remains a challenge.\\

\begin{figure}[ht!]
\vspace{-2em}
  \centering
   \includegraphics[trim={0, 0, 0, 0cm}, clip, width=0.7\linewidth]{result_tbl/syn_results.pdf}
   \caption{\textbf{Comparison of reconstruction quality across ground/aerial/satellite.}: We report PSNR$\uparrow$ and DreamSim$\downarrow$ (lower is better). All methods benefit from increased camera density. 2DGS consistently achieves the best perceptual quality. 
  }
   \label{fig:dreamsim}
   \vspace{-1em}
 \end{figure}


\noindent \textbf{2D-GS consistently gives best rendering results across ground/aerial/satellite:} Earlier, we noticed that VGGT obtained the \textit{best} performance out of all localization methods. We use VGGT zero-shot predicted poses, to initialize various gaussian splatting methods (2DGS, 3DGS and 3DGS-MCMC). We evaluate performance as number of input views increases from $D_1 \rightarrow D_2\rightarrow D_4$. The scaling-law (slope) suggests that 2D-Gaussian splatting consistently performs better. 

\textbf{Adding Real images harms rendering and yields noisy reconstructions:} 
Tab.~\ref{tab:psnr_dreamsim} shows that introducing real images into the training mix consistently degrades rendering quality across GS types and viewpoints.
Real-world lighting variation, sensor noise, clutter, and textures absent from synthetic data create a strong domain mismatch, making it difficult for the model to blend real and synthetic imagery.

Fig.~\ref{fig:synthesis_results} shows that increasing density from D1 to D4 produces sharper contours and more complete details, while mixing in 30 aerial and 30 ground real images at D2 introduces noise and domain mismatch, especially in ground views where real features absent from synthetic data begin to appear.





\begin{table}[t]
\centering
\caption{Rendering results across synthetic and real-image setups. We report PSNR and DreamSim for each GS type (2DGS, 3DGS, 3DGS\textsubscript{\tiny MCMC}) across aerial, street, and satellite viewpoints.}
\label{tab:psnr_dreamsim}
\setlength{\tabcolsep}{1.5pt}
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l l ccc ccc}
\toprule
& & \multicolumn{3}{c}{PSNR $\uparrow$} & \multicolumn{3}{c}{DreamSim $\downarrow$} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
Data & GS Type & Aerial & Ground & Satellite & Aerial & Ground & Satellite \\
\midrule
\multirow{3}{*}{Synthetic}
    & 2D                    & 12.1 & 14.9 & 13.0 & 0.49 & 0.26 & 0.19 \\
    & 3D                    & 11.8 & 14.7 & 13.0 & 0.52 & 0.31 & 0.17 \\
    & 3D\textsubscript{\tiny MCMC}
                              & 12.5 & 15.0 & 13.3 & 0.53 & 0.29 & 0.21 \\
\midrule
\multirow{3}{*}{Syn+Real}
    & 2D                    & 11.1 & 13.9 & 12.6 & 0.61 & 0.40 & 0.26 \\
    & 3D                    & 11.1 & 13.4 & 12.6 & 0.64 & 0.46 & 0.28 \\
    & 3D\textsubscript{\tiny MCMC}
                              & 11.2 & 12.8 & 13.4 & 0.79 & 0.71 & 0.68 \\
\bottomrule
\vspace{-3em}
\end{tabular}
}
\end{table}


\begin{figure*}[t!]
    \vspace{-2em}
    \centering
    \includegraphics[width=\textwidth]{figs/synthesis_results.png}
    \caption{
        Rendering results across satellite, aerial, and ground viewpoints.
        Each row shows a different view, with the leftmost column showing the ground-truth (GT) image followed by model renderings (R).
        From D1 to D4, the input density increases, and real images are incorporated with D2, introducing additional noise and domain mismatch.
        In particular, the ground-view renderings in D2 + Real contain real-image features that do not exist in the synthetic input distribution, highlighting the challenge of mixing synthetic and real sources.
    }
    \label{fig:synthesis_results}
\end{figure*}



\begin{table*}[ht!]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\caption{\textbf{Localization results across Ground+Aerial+Satellite setup.}
ZS = Zero-Shot, A-MD = Aerial-MegaDepth. RRA@5 / RTA@5 measure rotation / translation accuracy within 5° / 5 m. RRA Avg and RTA Avg denote mean performance across all domains.}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} & \textbf{Data} &
\multicolumn{2}{c}{\textbf{Ground}} &
\multicolumn{2}{c}{\textbf{Satellite}} &
\multicolumn{2}{c}{\textbf{Aerial}} &
\multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 &  & RRA@5 & RTA@5 & RRA@5 & RTA@5 & RRA@5 & RTA@5 & RRA & RTA \\
\midrule
Dust3r & ZS & 28.5\textsubscript{\tiny$\pm$0.71} & 21.6\textsubscript{\tiny$\pm$0.53} & 90.0\textsubscript{\tiny$\pm$1.92} & 39.9\textsubscript{\tiny$\pm$0.84} & 58.3\textsubscript{\tiny$\pm$1.37} & 44.3\textsubscript{\tiny$\pm$1.18} & 58.9\textsubscript{\tiny$\pm$1.23} & 35.3\textsubscript{\tiny$\pm$0.79} \\
Mast3r & ZS & 36.4\textsubscript{\tiny$\pm$0.86} & 29.6\textsubscript{\tiny$\pm$0.77} & 50.0\textsubscript{\tiny$\pm$1.04} & 13.3\textsubscript{\tiny$\pm$0.28} & 73.2\textsubscript{\tiny$\pm$1.49} & 68.9\textsubscript{\tiny$\pm$1.26} & 53.2\textsubscript{\tiny$\pm$1.07} & 37.3\textsubscript{\tiny$\pm$0.91} \\
VGGT & ZS & 75.1\textsubscript{\tiny$\pm$1.83} & 60.9\textsubscript{\tiny$\pm$1.29} & 66.6\textsubscript{\tiny$\pm$1.42} & 0.0\textsubscript{\tiny$\pm$0.00} & 79.2\textsubscript{\tiny$\pm$1.67} & 72.6\textsubscript{\tiny$\pm$1.23} & 73.6\textsubscript{\tiny$\pm$1.38} & 44.5\textsubscript{\tiny$\pm$0.95} \\
\hline
Dust3r & A-MD & 25.5\textsubscript{\tiny$\pm$0.64} & 23.2\textsubscript{\tiny$\pm$0.71} & 83.3\textsubscript{\tiny$\pm$1.78} & 29.9\textsubscript{\tiny$\pm$0.82} & 83.6\textsubscript{\tiny$\pm$1.74} & 64.8\textsubscript{\tiny$\pm$1.35} & 64.1\textsubscript{\tiny$\pm$1.27} & 39.3\textsubscript{\tiny$\pm$0.92} \\
Mast3r & A-MD & 29.1\textsubscript{\tiny$\pm$0.73} & 24.1\textsubscript{\tiny$\pm$0.61} & 96.6\textsubscript{\tiny$\pm$2.31} & 26.6\textsubscript{\tiny$\pm$0.68} & 77.0\textsubscript{\tiny$\pm$1.59} & 94.5\textsubscript{\tiny$\pm$2.18} & 67.6\textsubscript{\tiny$\pm$1.33} & 48.4\textsubscript{\tiny$\pm$0.97} \\
\hline
Dust3r & Sky2Ground & 32.4\textsubscript{\tiny$\pm$0.68} & 27.1\textsubscript{\tiny$\pm$0.63} & 79.4\textsubscript{\tiny$\pm$1.54} & 36.3\textsubscript{\tiny$\pm$0.87} & 83.8\textsubscript{\tiny$\pm$1.79} & 67.0\textsubscript{\tiny$\pm$1.16} & 65.2\textsubscript{\tiny$\pm$1.05} & 43.5\textsubscript{\tiny$\pm$0.94} \\
Mast3r & Sky2Ground & 33.2\textsubscript{\tiny$\pm$0.66} & 27.9\textsubscript{\tiny$\pm$0.59} & 81.0\textsubscript{\tiny$\pm$1.47} & 37.2\textsubscript{\tiny$\pm$0.81} & 85.1\textsubscript{\tiny$\pm$1.71} & 68.3\textsubscript{\tiny$\pm$1.12} & 69.4\textsubscript{\tiny$\pm$1.08} & 47.5\textsubscript{\tiny$\pm$0.89} \\
VGGT & Sky2Ground & 50.0\textsubscript{\tiny$\pm$1.25} & 46.1\textsubscript{\tiny$\pm$1.17} & 86.6\textsubscript{\tiny$\pm$1.94} & 53.3\textsubscript{\tiny$\pm$1.41} & 29.7\textsubscript{\tiny$\pm$0.61} & 31.5\textsubscript{\tiny$\pm$0.69} & 55.4\textsubscript{\tiny$\pm$1.09} & 43.6\textsubscript{\tiny$\pm$0.97} \\
\rowcolor{gray!20}
SkyNet & Sky2Ground & 76.7\textsubscript{\tiny$\pm$1.52} & 64.2\textsubscript{\tiny$\pm$1.27} & 88.9\textsubscript{\tiny$\pm$1.93} & 57.3\textsubscript{\tiny$\pm$1.14} & 84.0\textsubscript{\tiny$\pm$1.48} & 78.1\textsubscript{\tiny$\pm$1.06} & \textbf{83.2}\textsubscript{\tiny$\pm$1.37} & \textbf{66.5}\textsubscript{\tiny$\pm$0.98} \\
\bottomrule
\end{tabular}
\vspace{-6em}
}
\label{tab:gas_results}
\end{table*}

\subsection{Fine-Tuning-Analysis using Sky2Ground}
\label{sec:fine_tuning}
Earlier we noted that adding satellite during \textit{zero-shot inference} harms performance. In this section, we aim to study if \textit{simply adding} satellite during training, i.e. jointly fine-tuning existing models could work. To facilitate a systematic understanding, we first train on Ground-aerial (GA) data, and then on Ground/Aerial/Satellite data. Out of $51$ sites in Sky2Ground, we use $41$ for training, and remaining $10$ for evaluation.

\indent \textbf{Fine-Tuning with Ground-Aerial Data improves performance:} Tab \ref{tab:gas_results}, shows that training Dust3r on ground-aerial data improves on avg from $58.9\rightarrow 64.1 (RRA), 35.3 \rightarrow 39.3 (RTA)$. Similarly, Mast3r improves from $ 53.2 \rightarrow 67.6 (RRA), 37.3 \rightarrow 48.4 (RTA)$. Next, we study the effect of adding `satellite'.\\
\indent \textbf{Adding satellite improves `pairwise-view' nets like Dust3r/Mast3r} We note that adding satellite improves performance of nets like Dust3r/Mast3r from $64.1 \rightarrow 65.2 \text{ (RRA avg})$, $67.6 \rightarrow 69.4           \text{ (RTA avg)}$ respectively. A similar trend is observed for RTA. An inductive-bias common to \textit{both} Dust3r/Mast3r is that both process a \textit{pair of views} together, which \textit{might} explain this behaviour. However, choosing a pair out of $N$ total views requires $\binom{N}{2} \approx O(N^2)$ feed-forwards through the net, thereby making the entire pipeline \textit{extremely} slow. Next, we study the effect of adding `satellite' during training to \textit{single} feed-forward nets. \\
\indent \textbf{Adding satellite to `single-feedforward' nets like VGGT \textit{severely} hurts performance.}: In Tab\ref{tab:gas_results}, we observe that VGGT suffers a \textit{severe} drop, i.e. $73.6 \rightarrow 55.4$ (\textcolor{red}{-18.2\% RRA}), $44.5 \rightarrow 43.6$ (\textcolor{red}{-0.9\% RTA}). The above analysis leads to a \textit{counter-intuitive} insight. Adding satellite \textit{hurts} VGGT but not Dust3r/Mast3r. If extreme-distribution shift across ground/aerial/sat views \textit{were} the \textit{only} cause, we should have observed consistent-drops across \textit{all} methods. This leads us to question: \uline{`How can we further-improve  single-feedforward nets like VGGT?'}. Building upon VGGT makes sense because we can then \textit{bypass} classical SfM pipelines (aka COLMAP), global-alignment stage, and perform E2E optimization.

\vspace{-1em}
\section{Improving localization with satellite imagery}
As discussed in previous section \ref{sec:fine_tuning}, addition of satellite does not work even with fine-tuning. Inspired by this observation, here we present \textbf{SkyNet}, an architecture for cross-view camera localization. First, we formalize our problem statement and describe preliminaries.

\begin{figure*}
  \centering
  \vspace{-2em}
  \includegraphics[trim={0, 0, 0, 0cm}, clip, width=1\linewidth]{figs/arch.png}
  \caption{\textbf{SkyNet:} An architecture for cross-view camera localization. SkyNet consists of two encoders, 1) a Sat-Encoder processes input satellite images, and a GAS-Encoder processes ground/aerial/satellite views. Our model first patchifies the input images into tokens by DINO, and appends camera tokens for camera
prediction. GAS-encoder then alternates between self-attention and Masked-Satellite Attention. Camera/Depth heads collect satellite tokens from Sat-encoder, ground-aerial tokens from GAS-encoder and predict camera-poses and depth-maps respectively. 2) Masked-Satellite Attention \textit{restricts} aerial/ground from interacting with satellite modality. 3) Progressive-sampling gradually samples far-away cameras as training proceeds. 
  }
  \label{fig:skynet_v1}
  \vspace{-1.5em}
\end{figure*} 

\indent \textbf{Problem statement:} Given $N$ RGB images $I= \{ I_g, I_a, I_s\}_{N}$ consisting of $\{I_g\}$ ground-views, $\{I_a\}$ aerial-views and $\{I_s\}$ satellite-views, our objective is to predict the corresponding camera parameters $\{ \boldsymbol{g}_i \in \mathbb{R}^9\}^N_{i=1}$ and depth map $\{ D_i \in \mathbb{R}^{H \times W} \}^N_{i=1}$. Following VGGT\cite{wang2025vggt}, we represent $g_i$ in quaternion notation.  \\
\indent  \textbf{Preliminaries on VGGT:} Each of the $N$ input-images is first passed through a dino encoder. The resultant features are then concatenated with additional camera tokens $\mathbf{t}^{\boldsymbol{g}}_i \in \mathbb{R}^{1 \times C'}$ and four register tokens $\mathbf{t}^R_i \in \mathbb{R}^{4 \times C'}$. The camera/register tokens of first input view ($\mathbf{t}^{\boldsymbol{g}}_1 := \bar{\mathbf{t}}^{\boldsymbol{g}}, \ \mathbf{t}^R_1 := \bar{\mathbf{t}}^R$) are set to a \textit{different} set of learnable tokens $(\bar{\mathbf{t}}^{\boldsymbol{g}}, \bar{\mathbf{t}}^R)$ than those of all other frames ($\mathbf{t}^{\boldsymbol{g}}_i := \bar{\bar{\mathbf{t}}}^{\boldsymbol{g}}, \ \mathbf{t}^R_i := \bar{\bar{\mathbf{t}}}^R, \ i \in [2, \dots, N]$), which are also learnable.\\
\indent VGGT consists of $L$ layers of alternating frame-attention and global-attention. First, frame-attention allows tokens of each frame to interact among themselves. Next, in global-attention, information across different-views is aggregated, and aligned in the latent space. As in Sec\ref{sec:fine_tuning}, we notice two-issues with fine-tuning VGGT 1) It \textit{disturbs} the pre-trained VGGT weights, thereby losing the advantage of large-scale pre-training 2) Global Frame-attention \textit{forces} ground/aerial views to exchange information with satellite, but distribution-shift \textit{hurts} performance. 

\subsection{SkyNet}
Here we propose SkyNet, an architecture that processes input data in two parallel-streams. SkyNet consists of two components 1) a ground-aerial-sat (GAS)-encoder 2) a sat-encoder. \\
\indent \textbf{GAS-Encoder:} The Ground-Aerial-Satellite (GAS-encoder) consists of $L$ blocks. In each block, \textit{all} input views first undergo a self-attention. Next, we perform \textit{restricted-attention} termed as \uline{M}asked-\uline{S}atellite-\uline{A}ttention \textbf{(MSA)}. In Fig \ref{fig:skynet_v1}, MSA \textit{restricts}  \textit{ground/aerial} views  from interacting with \textit{sat}. However, \textit{sat} still interact with aerial/gnd views. The resulting attention values
$V = [v_G, v_A, v_S]$ are passed to $L-1$ identical blocks.  The self-attention, and MSA block are initialized with pre-trained VGGT weights, and kept-frozen. After each block, sat features $v_S$ are fed to the sat-encoder. \\
\indent \textbf{Sat-Encoder:} Given multiple satellite images $I_s$, we feed-forward them through a dino encoder. The output tokens first undergo a global-attention, where all the sat-views interact with each other, resulting in the latent $z$. Next, we update $z = z +v_s$, where $v_s$ are the refined \textit{sat} features coming from the GAS-encoder. \\
\indent \textbf{Camera/Depth-Map Predictions:} 
The camera parameters $(\hat{\boldsymbol{g}}^i)_{i=1}^N$ are predicted from the output camera tokens $({\hat{\mathbf{t}}}^\bg_i)_{i=1}^N$ using four additional self-attention layers followed by a linear layer. 
This camera-head decodes satellite-poses from the satellite-encoder, and aerial/ground poses from the GAS encoder. Additionally, we leverage a DPT head to output dense features $T_i \in \mathbb{R}^{C \times H \times W}$. Both camera/depth-head are \textit{shared} across GAS encoder/satellite encoder. \\
 \indent \textbf{Losses:} We set the number of transformer layers as $L=24$. We train SkyNet end-to-end via a multi-task loss 
$\mathcal{L} = \mathcal{L}_{\text{cam, sat}} + \alpha \mathcal{L}_{\text{cam, gnd/aerial}} + \mathcal{L}_{\text{depth}}$, where we empirically set $\alpha = 0.4$. 
The camera loss, depth loss, and other hyperparameters assume similar implementation/initialization as VGGT\cite{wang2025vggt}.


\begin{table*}[t!]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}
\begin{minipage}{0.48\linewidth}
\centering
\vspace{-15em}
\caption{\textbf{Localization results across Ground+Satellite setup.}
RRA@5 / RTA@5 denote rotation and translation accuracy within 5° / 5 m.
ZS = Zero-Shot.}
\vspace{-4em}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method} & \textbf{Data} &
\multicolumn{3}{c}{\textbf{Ground}} &
\multicolumn{3}{c}{\textbf{Satellite}} &
\textbf{Overall Avg} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 &  & RRA@5 & RTA@5 & Avg & RRA@5 & RTA@5 & Avg &  \\
\midrule
Dust3r & ZS & 29.2 & 19.1 & 24.2 & 90.0 & 56.6 & 73.3 & 48.7 \\
Mast3r & ZS & 32.8 & 31.5 & 32.2 & 73.3 & 33.3 & 53.3 & 42.7 \\
VGGT   & ZS & 70.2 & 61.6 & 65.9 & 76.6 & 3.3  & 40.0 & 52.9 \\
\midrule
VGGT   & Sky2Ground & 34.5 & 40.2 & 37.4 & 83.3 & 33.3 & 58.3 & 47.8 \\
\rowcolor{gray!20} 
\textbf{SkyNet} & \textbf{Sky2Ground} & 71.3 & 64.9 & 68.1 & 88.0 & 36.3 & 62.2 & \textbf{65.1} \\
\bottomrule
\vspace{-24em}
\end{tabular}
\label{tab:gs_results}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\centering
\caption{\textbf{Ablation of SkyNet variants.}
Effect of MSA (Masked Satellite Attention), CA-CS (Curriculum-Aware Camera Sampling), and P-VS (Progressive View-Sampling).}
\begin{tabular}{l|ccccc l}
\toprule
\textbf{Method} & \textbf{GAS-Enc.} & \textbf{Sat-Enc.} & \textbf{MSA} & \textbf{CA-CS} & \textbf{P-VS} & \textbf{Avg} \\
\midrule
VGGT (trained) & A+G+S & - & \xmark & \xmark & \xmark & 47.8 \\
\hline
VGGT-ZS        & A+G+S & - & \xmark & \xmark & \xmark & 52.9 \\
\hline
SkyNet (Ours)  & A+G & S & \xmark & \xmark & \xmark & 53.1 \textcolor{mypink}{0.2$\uparrow$}\\
               & A+G+S & S & \xmark & \xmark & \xmark & 53.8 \textcolor{mypink}{0.9$\uparrow$}\\
\cline{2-7}
               & A+G+S & S & \xmark & \checkmark & \xmark & 54.3 \textcolor{mypink}{1.4$\uparrow$}\\
               & A+G+S & S & \xmark & \xmark & \checkmark & 61.1 \textcolor{mypink}{7.3$\uparrow$}\\
               & A+G+S & S & \checkmark & \xmark & \xmark & 62.7 \textcolor{mypink}{8.2$\uparrow$}\\
\cline{2-7}
               & A+G+S & S & \checkmark & \checkmark & \xmark & 63.8 \textcolor{mypink}{10.9$\uparrow$}\\
               & A+G+S & S & \checkmark & \xmark & \checkmark & 64.9 \textcolor{mypink}{12.0$\uparrow$}\\
\cline{2-7}
\rowcolor{gray!20}
               & A+G+S & S & \checkmark & \checkmark & \checkmark & 
               65.1 \textcolor{mypink}{12.2$\uparrow$}\\
\bottomrule
\end{tabular}
\label{tab:skynet_ablation}
\end{minipage}

\end{table*}


\subsection{Cross-View Training strategies}
\indent As humans, we learn how to solve a particular problem by solving easier instances first, and gradually increasing the level of difficulty. This has been known as `curriculum-learning' in prior-literature. Inspired by this, we propose two training strategies for cross-view localization 1) \uline{C}urriculum \uline{A}ware \uline{C}amera-\uline{S}ampling (\textbf{CA-CS}), 2) \uline{P}rogressive-\uline{V}iew \uline{S}ampling \textbf{(P-VS)}.\\
 \indent \textbf{CA-CS sampling:}  During initial epochs, we sample cameras that lie closer to one other. As training proceeds, we gradually sample cameras far away from one another, for eg, non-overlapping cameras. Consider two-views with extrinsics $(R_1,R_2)$, and $(t_1, t_2)$. We estimate rotation/translation distance $d_R/d_T$ as:
\begin{equation}
d_R = \tfrac{1}{\pi}\arccos\!\left(\tfrac{\operatorname{Tr}(R_1^{\top}R_2)-1}{2}\right), \quad
d_T = \|t_1 - t_2\|_2,
\end{equation}
\noindent where, $D(I_1, I_2) = d_R + \lambda_t d_T$, where we set $\lambda_t = 0.5$, balances the rotation and translation terms. We pre-compute and cache pair-wise distances of all the cameras in a scene. For a given ground-view $I_1$, all the other views are sorted in increasing order of distance, and sampled with equal offset w.r.t each other. Our distance-metric doesn't involve explicit-point/feature-matching as in \cite{dust3r_cvpr24,mast3r_arxiv24}, and runs even on a CPU.\\
\indent \textbf{P-VS sampling:} Intuitively, \textit{ground/sat} views are extreme-viewpoints. However, aerial-images can serve as a `bridge' connecting these  modalities together\cite{vuong2025aerialmegadepth}. During training, we sample $N$ total images, where $N=N_a+N_g+N_s$ images, $N_a,N_g,N_s$ being number of ground/aerial/sat images. In beginning of our training schedule, we sample \textit{more number} of aerial-views $(N_a\approx N)$. Towards the end, we only retain ground/satellite images ($N_a\approx 0$). Therefore, our SkyNet gradually transitions from an easier problem, (localizing ground/aerial/sat views) to harder scenarios (ground/sat only).


\subsection{Results}

We evaluate SkyNet on \textit{dense2} setup, and consider \textit{both} ground/aerial/satellite , as well as ground/satellite setup. Note that ground/satellite is an \textit{extremely-realistic} scenario since aerial-imagery might not be available in certain-regions, for eg, forests, and war-zones.  We report both RRA@5 and RTA@5, with standard-deviation across $10$ sites in Sky2Ground. In Tab\ref{tab:gas_results}, we observe that SkyNet achieves a sota score of $83.2\%$(\textcolor{darkgreen}{+9.6\% RRA}), $83.2\%$(\textcolor{darkgreen}{+22.0\% RTA}). In Tab\ref{tab:gs_results}, we report $avg = (\frac{RRA@5 + RTA@5}{2})$. We observe our SkyNet improves VGGT even further to $65.1$ on average, marking improvement of (\textcolor{darkgreen}{+12.2\% }). 


\subsection{Ablations on SkyNet}
In Tab \ref{tab:skynet_ablation}, we discuss how different components in SkyNet perform in isolation w.r.t to each other. \\
\indent \textbf{Processing satellite along with aerial/ground images helps.} Processing \textit{sat} images in \textit{both} Ground-Aerial encoder, and Sat-encoder fares better than processing satellite only in Sat-encoder (+0.9 vs +0.2). \\
\indent \textbf{Masked Sat-Attention is the most contributing component:} In Tab\ref{tab:skynet_ablation}, using Masked-Sat attention results in highest increase of  $8.2$. Masking constraint ensures that satellite-tokens are refined by both ground/aerial tokens. Furthermore, we retain strong zero-shot performance of VGGT in ground/aerial case, since ground-aerial tokens \textit{never} interact with input satellite. \\
\indent \textbf{Progressive-View Sampling (P-VS) is the best training-strategy:} Training SkyNet with \textit{only} P-VS obtains $+7.3$, whereas with CA-CS only improves by $1.4$. This shows that decreasing aerial-views during training is the better strategy.\\
\indent \textbf{Adding satellite features from VGGT encoder$\rightarrow$ Sat-encoder outperforms naive cross-attention.} We perform an additional ablation, where instead of `adding' satellite-tokens from the Ground-Aerial encoder, we replace it with cross-attention\cite{carion2020end}. Avg performance \textit{drops} from $65.1$ to $59.7$, indicating that cross-attention is not the best choice.\\
\indent \textbf{SkyNet's improvements are not merely due to increasing-parameters:} We create a flop-matched baseline by increasing VGGT to additional $24$ layers. This ensures that parameter count becomes \textit{identical} to proposed SkyNet. The performance improves from $47.8$ to $50.4$. However, it still lies below VGGT's zero-shot performance $(52.9)$, as well as SkyNet's results $(65.1)$, indicating that improvements are not \textit{merely} due to increasing parameters, but due to MSA/CA-CS/P-VS components. \\
\section{Conclusion}
We introduced the problem of jointly localizing cameras across ground, aerial, and satellite views. We presented Sky2Ground, a dataset spanning both real and synthetic imagery, and showed that naïve fine-tuning of existing models is hindered primarily by the distribution shift introduced by satellite views. To address this, we proposed SkyNet, a cross-view extension of VGGT that leverages curriculum-inspired strategies such as progressive view and camera sampling. We sincerely hope that Sky2Ground may serve as a foundation for future research.\\

\noindent \textbf{Limitations:} Our method is inherently two-stage, in first-stage we predict-poses, and then rely on gaussian-splat for rendering. Exploring \textit{unified-models} capable of predicting poses/gaussian-parameters remains an interesting direction. \\


\noindent\textbf{Acknowledgments}
\label{sec:acknowledgments}
This work was supported by Intelligence Advanced Research Projects Activity (IARPA) via Department of Interior/Interior Business Center (DOI/IBC) contract number 140D0423C0074. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes, notwithstanding any copyright annotation thereon. Disclaimer: The views and
conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of IARPA, DOI/IBC, or the U.S. Government.


